Graph Augmentation for Cross Graph Domain Generalization

Cross-graph node classification, utilizing the abundant labeled nodes from one graph to help classify unlabeled nodes in another graph, can be viewed as a domain generalization problem of graph neural networks (GNNs) due to the structure shift commonly appearing among various graphs. Nevertheless, current endeavors for cross-graph node classification mainly focus on model training. Data augmentation approaches, a simple and easy-to-implement domain generalization technique, remain under-explored. In this paper, we develop a new graph structure augmentation for the crossgraph domain generalization problem. Specifically, low-weight edgedropping is applied to remove potential noise edges that may hinder the generalization ability of GNNs, stimulating the GNNs to capture the essential invariant information underlying different structures. Meanwhile, clustering-based edge-adding is proposed to generate invariant structures based on the node features from the same distribution. Consequently, with these augmentation techniques, the GNNs can maintain the domain invariant structure information that can improve the generalization ability. The experiments on out-ofdistribution citation network datasets verify our method achieves state-of-the-art performance among conventional augmentations.

==> images/graph_OOD.tex <==
\begin{figure*}[th]
    \centering

    \includegraphics[width=0.95\linewidth]{images/graph_OOD_.pdf}
    % \vspace{-1mm}
     \caption{Examples of different types of graph out-of-distribution data\cite{li2022ood} }% pseudo label $\hat{y}_i$ }
    \label{fig:graph_ood}
        % \vspace{2mm}
\end{figure*}

==> tables/tab_ab_study_edge_all.tex <==
 
 \begin{table}[ht]
\def\p{$\pm$} 
\centering
% \vspace{-2mm}
\caption{The comparison with different graph augmentations. The backbone is GIN. ( CD $\to$ A, A: ACM, D: DBLP, C: Citation)}
% \vspace{-0mm}
\scalebox{0.9}{
\begin{tabular}{c|c|ccc}
\toprule 
Methods & Augmenters  &  Micro F1 &  Macro F1 & Acc  \\
\midrule
\multirow{8}{*}{GIN}                     
&  baseline   &   56.45 $\pm$ 1.45 & 53.55 $\pm$ 2.64 & 83.04 $\pm$ 0.94    
% \cline{2-5}
 \\    
& only random edge &      61.55 $\pm$ 1.02 & 60.15 $\pm$ 1.33 & 85.72 $\pm$ 0.52                  
  \\  
& only clustering edge  &   \underline{69.23 $\pm$ 0.72} & 68.37 $\pm$ 0.99 & 86.80 $\pm$ 0.39     \\ 
% \cline{2-4}
 & random edge adding  &  61.54 $\pm$ 0.73 & 60.86 $\pm$ 0.84 & 86.14 $\pm$ 0.20                        
 \\                                       
& edge dropping &      64.72 $\pm$ 1.95 & 63.91 $\pm$ 2.22 & 85.63 $\pm$ 0.77   
\\
&  w/o clustering &      69.08 $\pm$ 0.82 & \underline{68.10 $\pm$ 1.28} & \underline{87.22 $\pm$ 0.49 }         
  \\                        
% \hline
 & w/o low weight dropping & 56.89 $\pm$ 3.33 &  52.50 $\pm$ 3.34 &  87.08 $\pm$ 0.63
\\
& low weigh dropping + clustering (ours) & \textbf{69.43 $\pm$ 0.65} & \textbf{68.77 $\pm$ 1.07} & \textbf{87.36 $\pm$ 0.34}
\\
\bottomrule
    \end{tabular}
    }
    % \vspace{-0mm}
    \label{tab:ab_study_edge}    
\end{table}

==> tables/tab_augmentations_ACD.tex <==
 
 \begin{table*}[ht]
\def\p{$\pm$} 
\centering
% \vspace{-2mm}
\caption{The comparison with different graph augmentations ( AC $\to$ D, A: ACM, D: DBLP, C: Citation)}
% \vspace{-0mm}
\scalebox{0.99}{
\begin{tabular}{c|c|ccc}
\toprule 
Methods & Augmenters  &  Micro F1 &  Macro F1 & Acc  \\
\midrule
% \hline
\multirow{7}{*}{GIN}                       
&  baseline   & 63.73 $\pm$ 1.31 & 58.63 $\pm$ 2.41 & 86.54 $\pm$ 0.41                                 
 \\                                            
& edge dropping & 71.19 $\pm$ 0.99 & 68.28 $\pm$ 1.01 & 88.66 $\pm$ 0.51                       
  \\                                           
 & edge adding  & 67.83 $\pm$ 0.49 & 64.71 $\pm$ 1.04 & 88.53 $\pm$ 0.18                          
 \\                                            
& feature masking & 71.31 $\pm$ 0.37 & 68.28 $\pm$ 0.65 & \textbf{89.46 $\pm$ 0.12}                            
  \\                                           
 & feature dropout &     70.11 $\pm$ 0.98 & 65.88 $\pm$ 1.88 & \underline{89.43 $\pm$ 0.27}                       
  \\   
  
&  Low weight dropping (ours) & \textbf{ 72.55 $\pm$ 0.60} & \underline{69.61 $\pm$ 1.22} & 88.54 $\pm$ 0.30  \\
&  Low weight + clustering (ours)     & \underline{72.46 $\pm$ 0.78} & \textbf{70.05 $\pm$ 1.71} & 88.52 $\pm$ 0.41     
  \\                                           
\bottomrule
    \end{tabular}
    }
    % \vspace{-0mm}
    \label{tab:augmentation_ACD}    
\end{table*}

==> tables/tab_augmentations_ADC.tex <==
 
 \begin{table*}[ht]
\def\p{$\pm$} 
\centering
% \vspace{-2mm}
\caption{The comparison with different graph augmentations ( AD $\to$ C, A: ACM, D: DBLP, C: Citation)}
% \vspace{-0mm}
\scalebox{0.95}{
\begin{tabular}{c|c|ccc}
\toprule 
Methods & Augmenters  &  Micro F1 &  Macro F1 & Acc  \\
\midrule

\multirow{7}{*}{GIN} &  baseline & 63.02 $\pm$ 1.31 & 56.55 $\pm$ 1.65 & 86.35 $\pm$ 0.62                  
 \\                          
& edge dropping     & {70.67 $\pm$ 1.24} & 67.55 $\pm$ 1.60 & 88.46 $\pm$ 0.43         
  \\                         
 & edge adding   & 69.04 $\pm$ 0.65 & 65.32 $\pm$ 0.78 & 88.88 $\pm$ 0.24                
 \\
& feature masking   & 72.17 $\pm$ 0.76 & 68.11 $\pm$ 1.17 & \underline{89.66 $\pm$ 0.23}          
  \\                         
 & feature dropout  & 70.14 $\pm$ 1.60 & 63.20 $\pm$ 2.54 & 89.69 $\pm$ 0.43         
  \\                         
&  Low weight dropping (ours) &  \underline{73.45 $\pm$ 0.89} & \underline{70.04 $\pm$ 1.27} & 89.23 $\pm$ 0.44 
  \\                      
  & low weight + clustering (ours) & \textbf{74.77 $\pm$ 0.60} & \textbf{71.79 $\pm$ 1.18} & \textbf{89.77 $\pm$ 0.30} \\
\bottomrule
    \end{tabular}
    }
    % \vspace{-0mm}
    \label{tab:tab:augmentation_ADC}    
\end{table*}

==> tables/tab_augmentations_CDA.tex <==
 
 \begin{table*}[ht]
\def\p{$\pm$} 
\centering
% \vspace{-2mm}
\caption{The comparison with different graph augmentations ( CD $\to$ A, A: ACM, D: DBLP, C: Citation)}
% \vspace{-0mm}
\scalebox{0.95}{
\begin{tabular}{c|c|ccc}
\toprule 
Methods & Augmenters  &  Micro F1 &  Macro F1 & Acc  \\
\midrule
% \hline
\multirow{7}{*}{GIN}                       
&  baseline   &   56.45 $\pm$ 1.45 & 53.55 $\pm$ 2.64 & 83.04 $\pm$ 0.94                               
 \\                                            
& edge dropping &      64.72 $\pm$ 1.95 & 63.91 $\pm$ 2.22 & 85.63 $\pm$ 0.77                  
  \\                                           
 & edge adding  &  61.54 $\pm$ 0.73 & 60.86 $\pm$ 0.84 & 86.14 $\pm$ 0.20                        
 \\                                            
& feature masking &  62.28 $\pm$ 1.99 & 60.47 $\pm$ 2.64 & 85.95 $\pm$ 0.61                          
  \\                                           
 & feature dropout &    61.53 $\pm$ 1.04 & 59.64 $\pm$ 1.44 & 85.90 $\pm$ 0.38                        
  \\                                           
&  Low weight dropping (ours) &      \underline{69.08 $\pm$ 0.82} & \underline{68.10 $\pm$ 1.28} & \underline{87.22 $\pm$ 0.49}           
  \\  
& Low weight + clustering (ours) & \textbf{69.43 $\pm$ 0.65} & \textbf{68.77 $\pm$ 1.07} & \textbf{87.36 $\pm$ 0.34} \\
\bottomrule
    \end{tabular}
    }
    % \vspace{-0mm}
    \label{tab:augmentation_CDA}    
\end{table*}

==> tables/tab_drop_norm_edge.tex <==
 
 \begin{table}[ht]
\def\p{$\pm$} 
\centering
% \vspace{-2mm}
\caption{The comparison between random edge dropping and low weight dropping. The backbone is GCN ( A: ACM, D: DBLP, C: Citation, SA: Spectral Augmentation)}
% \vspace{-0mm}
\scalebox{0.95}{
\begin{tabular}{c|ccc|ccc}
\toprule 
% \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{AD $\to$ C}    & \multicolumn{2}{c|}{AC $\to$ D}  & \multicolumn{2}{c}{CD $\to$ A} \\
\multirow{2}{*}{drop rate} & \multicolumn{3}{c|}{random}    & \multicolumn{3}{c}{low weights (ours)}  \\
 & Micro F1 &  Macro F1 & Acc & Micro F1 & Macro F1 & Acc \\
\midrule
0.0 & 63.66 $\pm$ 0.68 & 61.17 $\pm$ 0.84 & 85.71 $\pm$ 0.25  & 63.66 $\pm$ 0.68 & 61.17 $\pm$ 0.84 & 85.71 $\pm$ 0.25  \\                 
0.1 & 65.67 $\pm$ 0.83 &62.09 $\pm$ 0.73 & 87.37 $\pm$ 0.25 &   64.02 $\pm$ 0.60 & 61.47 $\pm$ 0.69 & 85.92 $\pm$ 0.23
  \\                 
0.2 &  66.33 $\pm$ 0.91 & \textbf{62.40 $\pm$ 1.01} & 87.82 $\pm$ 0.22 &  64.46 $\pm$ 0.76 & 61.67 $\pm$ 0.77 & 86.10 $\pm$ 0.29
  \\                       
0.3 & 66.60 $\pm$ 0.87 & 61.96 $\pm$ 1.04 & 88.12 $\pm$ 0.22  &  65.72 $\pm$ 0.58 & 62.80 $\pm$ 0.75 & 86.65  $\pm$ 0.22
  \\                       
0.4 & 66.61 $\pm$ 0.83 & 61.70 $\pm$ 1.09 & 88.28 $\pm$ 0.20 &  67.92 $\pm$ 0.45 & 64.86 $\pm$ 0.57 & 87.54 $\pm$ 0.22
  \\                        
0.5 &  66.66 $\pm$ 0.77 & 61.43 $\pm$ 0.86 & 88.40 $\pm$ 0.19 &    69.07 $\pm$ 0.43 & 65.13 $\pm$ 0.39 & 88.24 $\pm$ 0.15
  \\                                                           
0.6 &  66.34 $\pm$ 0.75 & 60.64 $\pm$ 0.72 & 88.44 $\pm$ 0.17  &  70.73 $\pm$ 0.56 & 66.14 $\pm$ 0.51 & 88.95 $\pm$ 0.16
   \\   
0.7 & 66.49 $\pm$ 0.66 & 60.65 $\pm$ 0.62 & 88.53  $\pm$  0.15  &  \textbf{71.62 $\pm$ 0.75} & \textbf{66.09 $\pm$ 0.56} & \textbf{89.69 $\pm$ 0.18}
   \\               
0.8 & 66.40 $\pm$ 0.57 & 60.48 $\pm$ 0.63 & 88.53  $\pm$ 0.14 &  70.72 $\pm$ 0.92 & 64.56 $\pm$ 0.76 & 89.47 $\pm$ 0.21
   \\    
0.9 & \textbf{67.26 $\pm$ 0.90} & 61.14 $\pm$ 0.86 & \textbf{88.70 $\pm$ 0.22}   &  70.72 $\pm$ 0.92 & 64.56 $\pm$ 0.76 & 89.47 $\pm$ 0.21
   \\  
% \midrule                                         
% GCN + SA(Ours) & &  &    &   &  &       \\
% GAT + SA(Ours) &   &  &    &   &  &       \\
% GIN + SA(Ours) & 66.89 & 65.51 &  86.96  &   &  &       \\
% SGC + SA(Ours) &  &  &    &   &  &       \\
\bottomrule
    \end{tabular}
    }
    % \vspace{-0mm}
    \label{tab:low_weight_edge_drop}    
\end{table}

==> tables/tab_drop_norm_gat.tex <==
 
 \begin{table}[ht]
\def\p{$\pm$} 
\centering
% \vspace{-2mm}
\caption{The comparison between random edge dropping and low weight dropping. The backbone is GAT ( AD $\to$ C, A: ACM, D: DBLP, C: Citation)}
% \vspace{-0mm}
\scalebox{0.95}{
\begin{tabular}{c|ccc|ccc}
\toprule 
\multirow{2}{*}{drop rate} & \multicolumn{3}{c|}{random}    & \multicolumn{3}{c}{low weights (ours)}  \\
 & Micro F1 &  Macro F1 & Acc & Micro F1 & Macro F1 & Acc \\
\midrule
0.0  &  60.61 $\pm$ 1.18 & 56.84 $\pm$ 1.29 & 85.87 $\pm$ 0.3 &
 \\  
0.1 &  63.76 $\pm$ 0.97 & 59.63 $\pm$ 1.14 & 86.84 $\pm$ 0.31 &
  \\  
0.2 &  
  \\  
0.3 &  
  \\  
0.4 &  
  \\  
0.5 &  
  \\  
0.6 &  
   \\  
0.7 &  
   \\  
0.8 &  
   \\  
0.9 &  
\\
\bottomrule
    \end{tabular}
    }
    % \vspace{-0mm}
    \label{tab:low_weight_edge_drop_gat}    
\end{table}

==> tables/tab_drop_norm_gin.tex <==
 
 \begin{table}[ht]
\def\p{$\pm$} 
\centering
% \vspace{-2mm}
\caption{The comparison between random edge dropping and low weight dropping. The backbone is GIN ( AD $\to$ C, A: ACM, D: DBLP, C: Citation, SA: Spectral Augmentation)}
% \vspace{-0mm}
\scalebox{0.95}{
\begin{tabular}{c|ccc|ccc}
\toprule 
% \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{AD $\to$ C}    & \multicolumn{2}{c|}{AC $\to$ D}  & \multicolumn{2}{c}{CD $\to$ A} \\
\multirow{2}{*}{drop rate} & \multicolumn{3}{c|}{random}    & \multicolumn{3}{c}{low weights (ours)}  \\
 & Micro F1 &  Macro F1 & Acc & Micro F1 & Macro F1 & Acc \\
\midrule
0.0 &   63.02 $\pm$ 1.31 & 56.55 $\pm$ 1.65 & 86.35 $\pm$ 0.62 & 63.02 $\pm$ 1.31 & 56.55 $\pm$ 1.65 & 86.35 $\pm$ 0.62 
 \\     
0.1 &  66.55 $\pm$ 0.85 & 61.91 $\pm$ 1.45 & 87.12 $\pm$ 0.48 & 64.38 $\pm$ 1.23 & 59.11 $\pm$ 2.53 & 86.15 $\pm$ 0.50 
  \\    
0.2 &   68.10 $\pm$ 0.63 & 64.24 $\pm$ 0.90 & 87.60 $\pm$ 0.30 & 65.90 $\pm$ 1.38 & 61.74 $\pm$ 2.00 & 86.48 $\pm$ 0.56
  \\    
0.3 &   68.77 $\pm$ 0.97 & 65.09 $\pm$ 1.78 & 88.00 $\pm$ 0.35 & 66.71 $\pm$ 0.58 & 61.70 $\pm$ 2.03 & 86.84 $\pm$ 0.39 
  \\    
0.4 &   69.66 $\pm$ 1.59 & 66.01 $\pm$ 1.64 & 88.40 $\pm$ 0.66 & 68.72 $\pm$ 1.16 & 64.70 $\pm$ 2.49 & 87.43  $\pm$ 0.37
  \\    
0.5 &   70.43 $\pm$ 1.31 & 67.20 $\pm$ 1.08 & 88.64 $\pm$ 0.54 &  70.18 $\pm$ 1.25 & 66.41 $\pm$ 1.70 & 87.84  $\pm$ 0.53

  \\    
0.6 &   70.59 $\pm$ 1.83 & 67.30 $\pm$ 1.40 & \textbf{88.65 $\pm$ 0.74} &  70.50 $\pm$ 1.43 & 67.01 $\pm$ 1.93 & 87.90  $\pm$ 0.64

   \\   
0.7 &  70.58 $\pm$ 1.64 & \textbf{67.71 $\pm$ 1.41} & 88.54 $\pm$ 0.66 & 72.25 $\pm$ 1.28 & 68.96 $\pm$ 1.85 & 88.61 $\pm$ 0.61
   \\   
0.8 & \textbf{70.67 $\pm$ 1.24} & 67.55 $\pm$ 1.60 & 88.46 $\pm$ 0.43 &  \textbf{73.45 $\pm$ 0.89} & \textbf{70.04 $\pm$ 1.27} & \textbf{89.23 $\pm$ 0.44}
   \\   
0.9 &   69.92 $\pm$ 1.80 & 66.17 $\pm$ 3.96 & 87.91  $\pm$ 0.81 & 73.45 $\pm$ 0.89 & 70.04 $\pm$ 1.27 & 89.23  $\pm$ 0.44
   \\  
\bottomrule
    \end{tabular}
    }
    % \vspace{-0mm}
    \label{tab:low_weight_edge_drop_gin}    
\end{table}
